Brighteye: Glaucoma Screening with Color Fundus Photographs based on Vision Transformer

Differences in image quality, lighting conditions, and patient demographics pose challenges to automated glaucoma detection from color fundus photography. Brighteye, a method based on Vision Transformer, is proposed for glaucoma detection and glaucomatous feature classification. Brighteye learns long-range relationships among pixels within large fundus images using a self-attention mechanism. Prior to being input into Brighteye, the optic disc is localized using YOLOv8, and the region of interest (ROI) around the disc center is cropped to ensure alignment with clinical practice. Optic disc detection improves the sensitivity at 95% specificity from 79.20% to 85.70% for glaucoma detection and the Hamming distance from 0.2470 to 0.1250 for glaucomatous feature classification. In the developmental stage of the Justified Referral in AI Glaucoma Screening (JustRAIGS) challenge, the overall outcome secured the fifth position out of 226 entries.

==> refs.tex <==

@article{lin2023stenunet,
  title={StenUNet: Automatic Stenosis Detection from X-ray Coronary Angiography},
  author={Lin, Hui and Liu, Tom and Katsaggelos, Aggelos and Kline, Adrienne},
  journal={arXiv preprint arXiv:2310.14961},
  year={2023}
}
@article{lin2019automated,
  title={Automated defect inspection of LED chip using deep convolutional neural network},
  author={Lin, Hui and Li, Bin and Wang, Xinggang and Shu, Yufeng and Niu, Shuanglong},
  journal={Journal of Intelligent Manufacturing},
  volume={30},
  pages={2525--2534},
  year={2019},
  publisher={Springer}
}


@article{liu2023yolo,
  title={YOLO-Angio: An Algorithm for Coronary Anatomy Segmentation},
  author={Liu, Tom and Lin, Hui and Katsaggelos, Aggelos K and Kline, Adrienne},
  journal={arXiv preprint arXiv:2310.15898},
  year={2023}
}
@article{mao2023deep,
  title={A deep learning framework for layer-wise porosity prediction in metal powder bed fusion using thermal signatures},
  author={Mao, Yuwei and Lin, Hui and Yu, Christina Xuan and Frye, Roger and Beckett, Darren and Anderson, Kevin and Jacquemetton, Lars and Carter, Fred and Gao, Zhangyuan and Liao, Wei-keng and others},
  journal={Journal of Intelligent Manufacturing},
  volume={34},
  number={1},
  pages={315--329},
  year={2023},
  publisher={Springer}
}
@inproceedings{niu2019defectgan,
  title={DefectGAN: Weakly-supervised defect detection using generative adversarial network},
  author={Niu, Shuanlong and Lin, Hui and Niu, Tongzhi and Li, Bin and Wang, Xinggang},
  booktitle={2019 IEEE 15th international conference on automation science and engineering (CASE)},
  pages={127--132},
  year={2019},
  organization={IEEE}
}
@inproceedings{wang2022workflow,
  title={A workflow for computer-aided diagnosis of glaucoma},
  author={Wang, He and Sun, Hongyi and Fang, Yi and Li, Shuo and Feng, Ming and Wang, Renzhi},
  booktitle={2022 IEEE International Symposium on Biomedical Imaging Challenges (ISBIC)},
  pages={1--4},
  year={2022},
  organization={IEEE}
}
@inproceedings{khader2022elevating,
  title={Elevating fundoscopic evaluation to expert level-automatic glaucoma detection using data from the airogs challenge},
  author={Khader, Firas and Haarburger, Christoph and Kirr, J{\"o}rg-Christian and Menke, Marcel and Kather, Jakob Nikolas and Stegmaier, Johannes and Kuhl, Christiane and Nebelung, Sven and Truhn, Daniel},
  booktitle={2022 IEEE international symposium on biomedical imaging challenges (ISBIC)},
  pages={1--4},
  year={2022},
  organization={IEEE}
}
@article{aimyshev2022glaucoma,
  title={Glaucoma Detection Algorithm for the Artificial Intelligence for Robust Glaucoma Screening Challenge},
  author={Aimyshev, Temirgali and Eleusiz, Kanat},
  journal={AIROGS. pdf},
  year={2022}
}
@article{de2023airogs,
  title={AIROGS: artificial intelligence for robust glaucoma screening challenge},
  author={De Vente, Coen and Vermeer, Koenraad A and Jaccard, Nicolas and Wang, He and Sun, Hongyi and Khader, Firas and Truhn, Daniel and Aimyshev, Temirgali and Zhanibekuly, Yerkebulan and Le, Tien-Dung and others},
  journal={IEEE transactions on medical imaging},
  year={2023},
  publisher={IEEE}
}
@inproceedings{yu2021mil,
  title={Mil-vt: Multiple instance learning enhanced vision transformer for fundus image classification},
  author={Yu, Shuang and Ma, Kai and Bi, Qi and Bian, Cheng and Ning, Munan and He, Nanjun and Li, Yuexiang and Liu, Hanruo and Zheng, Yefeng},
  booktitle={Medical Image Computing and Computer Assisted Intervention--MICCAI 2021: 24th International Conference, Strasbourg, France, September 27--October 1, 2021, Proceedings, Part VIII 24},
  pages={45--54},
  year={2021},
  organization={Springer}
}

@software{yolov8_ultralytics,
  author = {Glenn Jocher and Ayush Chaurasia and Jing Qiu},
  title = {Ultralytics YOLOv8},
  version = {8.0.0},
  year = {2023},
  url = {https://github.com/ultralytics/ultralytics},
  orcid = {0000-0001-5950-6979, 0000-0002-7603-6750, 0000-0003-3783-7069},
  license = {AGPL-3.0}
}
@inproceedings{das2016detection,
  title={Detection of glaucoma using Neuroretinal Rim information},
  author={Das, Pranjal and Nirmala, SR and Medhi, Jyoti Prakash},
  booktitle={2016 International Conference on Accessibility to Digital World (ICADW)},
  pages={181--186},
  year={2016},
  organization={IEEE}
}
@article{sanfilippo2010geometric,
  title={A geometric morphometric assessment of the optic cup in glaucoma},
  author={Sanfilippo, Paul G and Cardini, Andrea and Sigal, Ian A and Ruddle, Jonathan B and Chua, Brian E and Hewitt, Alex W and Mackey, David A},
  journal={Experimental eye research},
  volume={91},
  number={3},
  pages={405--414},
  year={2010},
  publisher={Elsevier}
}
@article{hayreh1972optic,
  title={Optic disc changes in glaucoma.},
  author={Hayreh, SOHAN SINGH},
  journal={The British journal of ophthalmology},
  volume={56},
  number={3},
  pages={175},
  year={1972},
  publisher={BMJ Publishing Group}
}
@article{dosovitskiy2021image,
      title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale}, 
      author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
      year={2021},
      journal={arXiv preprint arXiv:2010.11929}
}
@article{lemij2023characteristics,
  title={Characteristics of a large, labeled data set for the training of artificial intelligence for glaucoma screening with fundus photographs},
  author={Lemij, Hans G and de Vente, Coen and S{\'a}nchez, Clara I and Vermeer, Koen A},
  journal={Ophthalmology Science},
  volume={3},
  number={3},
  pages={100300},
  year={2023},
  publisher={Elsevier}
}
@article{phene2019deep,
  title={Deep learning and glaucoma specialists: the relative importance of optic disc features to predict glaucoma referral in fundus photographs},
  author={Phene, Sonia and Dunn, R Carter and Hammel, Naama and Liu, Yun and Krause, Jonathan and Kitade, Naho and Schaekermann, Mike and Sayres, Rory and Wu, Derek J and Bora, Ashish and others},
  journal={Ophthalmology},
  volume={126},
  number={12},
  pages={1627--1639},
  year={2019},
  publisher={Elsevier}
}
@article{septiarini2015automatic,
  title={AUTOMATIC GLAUCOMA DETECTION BASED ON THE TYPE OF FEATURES USED: A REVIEW.},
  author={Septiarini, Anindita and Harjoko, Agus},
  journal={Journal of Theoretical \& Applied Information Technology},
  volume={72},
  number={3},
  year={2015}
}
@article{zedan2023automated,
  title={Automated glaucoma screening and diagnosis based on retinal fundus images using deep learning approaches: A comprehensive review},
  author={Zedan, Mohammad JM and Zulkifley, Mohd Asyraf and Ibrahim, Ahmad Asrul and Moubark, Asraf Mohamed and Kamari, Nor Azwan Mohamed and Abdani, Siti Raihanah},
  journal={Diagnostics},
  volume={13},
  number={13},
  pages={2180},
  year={2023},
  publisher={MDPI}
}
@article{hemelings2023generalizable,
  title={A generalizable deep learning regression model for automated glaucoma screening from fundus images},
  author={Hemelings, Ruben and Elen, Bart and Schuster, Alexander K and Blaschko, Matthew B and Barbosa-Breda, Jo{\~a}o and Hujanen, Pekko and Junglas, Annika and Nickels, Stefan and White, Andrew and Pfeiffer, Norbert and others},
  journal={NPJ digital medicine},
  volume={6},
  number={1},
  pages={112},
  year={2023},
  publisher={Nature Publishing Group UK London}
}
@article{hemelings2021deep,
  title={Deep learning on fundus images detects glaucoma beyond the optic disc},
  author={Hemelings, Ruben and Elen, Bart and Barbosa-Breda, Jo{\~a}o and Blaschko, Matthew B and De Boever, Patrick and Stalmans, Ingeborg},
  journal={Scientific Reports},
  volume={11},
  number={1},
  pages={20313},
  year={2021},
  publisher={Nature Publishing Group UK London}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{lin2024usformer,
  title={Usformer: A Small Network for Left Atrium Segmentation of 3D LGE MRI},
  author={Lin, Hui and L{\'o}pez-Tapia, Santiago and Schiffers, Florian and Wu, Yunan and Gunasekaran, Suvai and Hwang, Julia and Bishara, Dima and Kholmovski, Eugene and Elbaz, Mohammed and Passman, Rod S and others},
  journal={Heliyon},
  year = {2024},
  issn = {2405-8440},
  publisher={Elsevier}
}
@article{nawaz2022efficient,
  title={An efficient deep learning approach to automatic glaucoma detection using optic disc and optic cup localization},
  author={Nawaz, Marriam and Nazir, Tahira and Javed, Ali and Tariq, Usman and Yong, Hwan-Seung and Khan, Muhammad Attique and Cha, Jaehyuk},
  journal={Sensors},
  volume={22},
  number={2},
  pages={434},
  year={2022},
  publisher={MDPI}
}
@article{buisson2021deep,
  title={Deep learning versus ophthalmologists for screening for glaucoma on fundus examination: A systematic review and meta-analysis},
  author={Buisson, Mathieu and Navel, Valentin and Labb{\'e}, Antoine and Watson, Stephanie L and Baker, Julien S and Murtagh, Patrick and Chiambaretta, Fr{\'e}d{\'e}ric and Dutheil, Fr{\'e}d{\'e}ric},
  journal={Clinical \& Experimental Ophthalmology},
  volume={49},
  number={9},
  pages={1027--1038},
  year={2021},
  publisher={Wiley Online Library}
}
@article{manzari2023medvit,
  title={MedViT: a robust vision transformer for generalized medical image classification},
  author={Manzari, Omid Nejati and Ahmadabadi, Hamid and Kashiani, Hossein and Shokouhi, Shahriar B and Ayatollahi, Ahmad},
  journal={Computers in Biology and Medicine},
  volume={157},
  pages={106791},
  year={2023},
  publisher={Elsevier}
}
@INPROCEEDINGS{Fousia2016,
  author={Shamsudeen, Fousia M and Raju, G.},
  booktitle={2016 International Conference on Next Generation Intelligent Systems (ICNGIS)}, 
  title={Enhancement of fundus imagery}, 
  year={2016},
  volume={},
  number={},
  pages={1-5},
  keywords={Histograms;Mathematical model;Image color analysis;Optical imaging;Integrated optics;Retina;Next generation networking;Fundus camera;fundus image;contrast enhancement;contrast limited adaptive histogram equalization},
  doi={10.1109/ICNGIS.2016.7854022}}
@inproceedings{wang2022using,
  title={Using Multi-Resolution Data to Accelerate Neural Network Training in Scientific Applications},
  author={Wang, Kewei and Lee, Sunwoo and Balewski, Jan and Sim, Alex and Nugent, Peter and Agrawal, Ankit and Choudhary, Alok and Wu, Kesheng and Liao, Wei-Keng},
  booktitle={2022 22nd IEEE International Symposium on Cluster, Cloud and Internet Computing (CCGrid)},
  pages={404--413},
  year={2022},
  organization={IEEE}
}
@article{madadi2024domain,
  title={Domain Adaptation-Based deep learning model for forecasting and diagnosis of glaucoma disease},
  author={Madadi, Yeganeh and Abu-Serhan, Hashem and Yousefi, Siamak},
  journal={Biomedical Signal Processing and Control},
  volume={92},
  pages={106061},
  year={2024},
  publisher={Elsevier}
}


